Synthetic data, real errors: how (not) to publish and use synthetic data

Generating synthetic data through generative models is gaining interest in the ML community and beyond, promising a future where datasets can be tailored to individual needs. Unfortunately, synthetic data is usually not perfect, resulting in potential errors in downstream tasks. In this work we explore how the generative process affects the downstream ML task. We show that the naive synthetic data approach -- using synthetic data as if it is real -- leads to downstream models and analyses that do not generalize well to real data. As a first step towards better ML in the synthetic data regime, we introduce Deep Generative Ensemble (DGE) -- a framework inspired by Deep Ensembles that aims to implicitly approximate the posterior distribution over the generative process model parameters. DGE improves downstream model training, evaluation, and uncertainty quantification, vastly outperforming the naive approach on average. The largest improvements are achieved for minority classes and low-density regions of the original data, for which the generative uncertainty is largest.

==> legacy_guidelines.tex <==
% \begin{table*}[]
% \tiny
% \begin{tabularx}{\textwidth}{
% >{\columncolor[HTML]{EA6B66}}X
% >{\columncolor[HTML]{7EA6E0}}X }
% {\color[HTML]{FFFFFF} \textbf{Synthetic data publisher}} &
%   {\color[HTML]{FFFFFF} \textbf{Synthetic data user}} \\
% {\color[HTML]{FFFFFF} \textit{} Generating multiple synthetic datasets using DGE aids downstream ML, even if the number of generated datasets is small (e.g. $K=5$).} &
%   {\color[HTML]{FFFFFF} \textit{(1)} Training models on an ensemble of synthetic datasets---either by training separate models and averaging predictions, or simply concatenating datasets---improves model performance on real data.} \\
% {\color[HTML]{FFFFFF} \textit{(2)} These datasets need to be distinguishable---i.e. publishing each set in separate files or create a variable that denotes the set---since for some downstream tasks (e.g. uncertainty quantification) it does not suffice to simply concatenate datasets without specifying the source of each sample.} &
%   {\color[HTML]{FFFFFF} \textit{(2)} Train-test-splits do not work naively on synthetic data, since this induces bias through evaluating on data from the same generative model. Instead, one can split on the synthetic dataset level: train on some synthetic datasets, and evaluate on others. Similarly,} \\
% {\color[HTML]{FFFFFF} \textit{(3)} DGE allows different generative model classes, e.g. GAN or VAE.} &
%   {\color[HTML]{FFFFFF} \textit{(3)} model selection using the naive approach is biased to select models with higher complexity, which can copy the generative model's learnt label distribution. This too is avoided by evaluating across different datasets.} \\
% {\color[HTML]{FFFFFF} \textit{(4)} Generating more synthetic data than real data is not necessarily a good idea, as this can lead to overconfident downstream models when users are not careful.} &
%   {\color[HTML]{FFFFFF} \textit{(4)} Uncertainty quantification in the synthetic data regime needs careful consideration, as naively estimating uncertainty using popular UQ methods (e.g. Deep Ensembles) do not consider uncertainty in the generative process itself. Here it helps to ensemble models trained on different synthetic datasets, since the difference between these models reflects generative uncertainty.} \\
% {\color[HTML]{FFFFFF} \textit{(5)} It is pertinent to include meta-data on the generative model, e.g. the amount of training data. Publishing the model class itself is also advisable, since the generative class can have implication on downstream model selection through congeniality.} &
%   {\color[HTML]{FFFFFF} \textit{(5)} Overfitting in the generative process exacerbates problems for the naive approach, when downstream models copy overfitted behaviour. } \\
% {\color[HTML]{FFFFFF} } &
%   {\color[HTML]{FFFFFF} \textit{(6)} The above implies that for regions with fewer samples it is especially important to use an ensemble approach, since the generative process is more likely to have overfitted samples in these regions.}

% \end{tabularx}
% \end{table*}
